Parallel Architecture and Hyperparameter Search via Successive Halving and Classification

We present a simple and powerful algorithm for parallel black box optimization called Successive Halving and Classification (SHAC). The algorithm operates in $K$ stages of parallel function evaluations and trains a cascade of binary classifiers to iteratively cull the undesirable regions of the search space. SHAC is easy to implement, requires no tuning of its own configuration parameters, is invariant to the scale of the objective function and can be built using any choice of binary classifier. We adopt tree-based classifiers within SHAC and achieve competitive performance against several strong baselines for optimizing synthetic functions, hyperparameters and architectures.

==> design.tex <==
\section{Design Decisions}

This section gives an overview of the various design decisions of the variant of SHAC used in our experiments and some interpretable ways to set them.

\subsection{Choice of classifier}
Internally, SHAC can use any binary classifier. In our experiments, we use gradient boosted trees~\cite{gboosting} to classify configurations at every stage. Although other classifier choices would be also possible, gradient boosted trees have shown to be powerful, robust to the choice to its own hyperparameters and easy to get working in new problem domains~\cite{xgboost}. Thankfully, gradient boosted trees are also extremely fast to train and perform inference on. We set the default number of trees in gradient boosting to 200 and do not change the default hyperparameters. We describe how the configurations sampled from each search space are encoded in the classifiers for every experiment in the corresponding sub-sections.

\subsection{Maximum number of classifiers}

If T is the total budget and W is the number of workers, the maximum number of classifiers is just $\frac{T}{W} - 1$. But, unfortunately the number of random proposals to generate a configuration also increases by a factor of 2 when a classifier is added to the SHAC cascade. So, additionally we cap the number of classifiers to a maximum value (described in each sub-section) so that the sampling does not become time-consuming. Although more efficient schemes than rejection sampling are possible, we did not explore them in this work.

\subsection{Minimum training set size}
Depending upon the total budget and the maximum number of classifiers that one can afford to set, we advocate setting a minimum training set size for each classifier. If $W$ is the number of workers, $T$ the total budget and $K$ be the maximum number of classifiers, then a reasonable default is to provide each classifier with at least ${W \lfloor \frac{T}{W(K + 1)} \rfloor}$ number of configurations. Additionally, after each classifier has been provided the minimum training set size number of points, we monitor the 5-fold cross validation accuracy to ensure each classifier has suitable predictive power. Once this is greater than 0.5, we add the classifier to the cascade and proceed to train the next classifier.

% With a higher budget, one can affford to have a higher training set size for each classifier.


